mT5: A massively multilingual pre-trained text-to-text transformer

The recent "Text-to-Text Transfer Transformer" (T5) leveraged a unified text-to-text format and scale to attain state-of-the-art results on a wide variety of English-language NLP tasks. In this paper, we introduce mT5, a multilingual variant of T5 that was pre-trained on a new Common Crawl-based dataset covering 101 languages. We detail the design and modified training of mT5 and demonstrate its state-of-the-art performance on many multilingual benchmarks. We also describe a simple technique to prevent "accidental translation" in the zero-shot setting, where a generative model chooses to (partially) translate its prediction into the wrong language. All of the code and model checkpoints used in this work are publicly available.

==> mt5 arxiv 031121/main_results.tex <==
\begin{table*}[t!]
\centering
%\begin{adjustbox}{scale=0.95,center}
\footnotesize
% Manually specify the width of the last column. Otherwise the last column is too wide.
\begin{tabular}{lccHcccp{7em}<{\centering\arraybackslash}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Sentence pair} & \multicolumn{2}{c}{Structured} & \multicolumn{3}{c}{Question answering} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8}
& XNLI & PAWS-X & POS & WikiAnn NER & XQuAD & MLQA & TyDiQA-GoldP \\
\midrule
Metrics & Acc. & Acc. & F1 & F1 & F1 / EM & F1 / EM & F1 / EM  \\
\midrule
\multicolumn{8}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tuned on English data only)}} \\
\midrule
mBERT          & 65.4 & 81.9 & 70.3 & 62.2 & 64.5 / 49.4 & 61.4 / 44.2 & 59.7 / 43.9 \\
XLM            & 69.1 & 80.9 & 70.1 & 61.2 & 59.8 / 44.3 & 48.5 / 32.6 & 43.6 / 29.1 \\
InfoXLM                  & 81.4 & - & - & - & - / - & 73.6 / 55.2 & - / - \\
X-STILTs & 80.4 & 87.7 & 74.4 & 64.7 & 77.2 / 61.3 & 72.3 / 53.5 & 76.0 / 59.5 \\
XLM-R  & 79.2 & 86.4 & 72.6 & 65.4 & 76.6 / 60.8 & 71.6 / 53.2 & 65.1 / 45.0 \\
%Anonymous & 80.0 & 87.9 & 74.9 & 64.0 & 78.7 / 63.3 & 72.4 / 53.7 & 81.3 / 68.5 \\ 
VECO & 79.9 & 88.7 & 75.1 & 65.7 & 77.3 / 61.8 & 71.7 / 53.2 & 67.6 / 49.1 \\
%FILTER & 83.62 & 91.42 & 76.2 & 67.66 & 82.42 / 68.01 & 76.22 / 57.73 & 71.73 / 55.15 \\
RemBERT & 80.8 & 87.5 & 76.5 & \textbf{70.1} & 79.6 / 64.0 & 73.1 / 55.0 & 77.0 / 63.0 \\
mT5-Small  & 67.5 & 82.4 & 72.6 & 50.5 & 58.1 / 42.5 & 54.6 / 37.1 & 35.2 / 23.2 \\
mT5-Base  & 75.4 & 86.4 & 72.6 & 55.7 & 67.0 / 49.0 & 64.6 / 45.0 & 57.2 / 41.2 \\
mT5-Large  & 81.1 & 88.9 & 72.6 & 58.5 & 77.8 / 61.5 & 71.2 / 51.7 & 69.9 / 52.2 \\
mT5-XL  & 82.9 & 89.6 & 72.6 & 65.5 & 79.5 / 63.6 & 73.5 / 54.5 & 75.9 / 59.4 \\
%mT5-XXL (75\% trained) & \scriptsize{\textbf{84.8}} & 89.2 & 72.6 & \scriptsize{\textbf{69.2}} & \scriptsize{\textbf{81.9 / 65.7}} & \scriptsize{\textbf{75.5 / 56.9}} & \scriptsize{\textbf{80.8 / 66.3}} \\
mT5-XXL  & \textbf{85.0} & \textbf{90.0} & 72.6 & 69.2 & \textbf{82.5 / 66.8} & \textbf{76.0 / 57.4} & \textbf{80.8 / 65.9} \\
\midrule
\multicolumn{8}{l}{\emph{Translate-train (models fine-tuned on English data plus translations in all target languages)}} \\
\midrule
%mBERT                    & 74.0 & 86.3 & -    & -    & 70.0 / 56.0 & 65.6 / 48.0 & 55.1 / 42.1 \\
%mBERT, multi-task        & 75.1 & 88.9 & -    & -    & 72.4 / 58.3 & 67.6 / 49.8 & 64.2 / 49.3 \\
XLM-R  & 82.6 & 90.4 &  -   & -    & 80.2 / 65.9 & 72.8 / 54.3 & 66.5 / 47.7 \\
%\midrule
%\textsc{Filter}                & 83.6   & 91.2 & 75.5 & 66.7 & 82.3 / 67.8  & 75.8 / 57.2 & 68.1 / 49.7 \\
\textsc{Filter} + Self-Teaching  & {83.9}   & 91.4 & 76.2 & - & {82.4} / {68.0}  & {76.2} / 57.7 & 68.3 / 50.9 \\
VECO & 83.0 & 91.1 & 75.1 & - & 79.9 / 66.3 & 73.1 / 54.9 & 75.0 / 58.9 \\
%T-ULRv2 + StableTune & 86.0 & \textbf{91.7} & 79.2 & 71.6 & 83.6 / 70.4 & 75.5 / 57.8 & 81.4 / 69.1 \\
%Polyglot & 84.2 & 91.3 & 77.5 & 68.3 & 79.1 / 64.8 & 72.7 / 54.6 & 74.4 / 58.8 \\
%MTDA & 83.6 & 91.4 & 76.2 & 67.7 & 82.4 / 68.0 & 76.2 / 57.7 & 71.7 / 55.1 \\
mT5-Small  & 64.7 & 79.9 & 72.6 & - & 64.3 / 49.5 & 56.6 / 38.8 & 48.2 / 34.0 \\
mT5-Base  & 75.9 & 89.3 & 72.6 & - & 75.3 / 59.7 & 67.6 / 48.5 & 64.0 / 47.7 \\
mT5-Large  & 81.8 & 91.2 & 72.6 & - & 81.2 / 65.9 & 73.9 / 55.2 & 71.1 / 54.9 \\
mT5-XL  & 84.8 & 91.0 & 72.6 & - & 82.7 / 68.1 & 75.1 / 56.6 & 79.9 / 65.3 \\
%mT5-XXL (75\% trained) & \scriptsize{\textbf{87.2}} & \scriptsize{\textbf{92.0}} & 72.6 & - & \scriptsize{\textbf{85.0 / 70.8}} & \scriptsize{\textbf{76.6} / \textbf{58.2}} & \scriptsize{\textbf{82.0 / 67.8}} \\
mT5-XXL  & \textbf{87.8} & \textbf{91.5} & 72.6 & - & \textbf{85.2 / 71.3} & \textbf{76.9 / 58.3} & \textbf{82.8 / 68.8} \\
\midrule
\multicolumn{8}{l}{\emph{In-language multitask (models fine-tuned on gold data in all target languages)}} \\
\midrule
mBERT & - & - & 91.5 & 89.1 & - & - & 77.6 / 68.0 \\
mT5-Small & - & - & - & 83.4 & - & - & 73.0 / 62.0 \\
mT5-Base & - & - & - & 85.4 & - & - & 80.8 / 70.0 \\
mT5-Large & - & - & - & 88.4 & - & - & 85.5 / 75.3 \\
mT5-XL & - & - & - & 90.9 & - & - & 87.5 / 78.1 \\
mT5-XXL & - & - & - & \textbf{91.2} & - & - & \textbf{88.5 / 79.1} \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\caption{Results on \textsc{xtreme} sentence-pair classification, structured prediction and question answering tasks. mBERT metrics are from \citet{hu2020xtreme}. Metrics for XLM, InfoXLM, X-STILTs and XLM-R are from \citet{fang2020filter}, though \citet{conneau2019unsupervised} report better performance of XLM-R on XNLI (80.9). All other metrics are from the original sources: \textsc{Filter} \cite{fang2020filter}, VECO \cite{luo2020veco} and RemBERT \cite{chung2020rethinking}. For the ``translate-train'' setting, we include English training data, so as to be comparable with \citet{fang2020filter} and \citet{luo2020veco}. This differs from the \textsc{xtreme} ``translate-train'' setup of \citet{hu2020xtreme}. For mT5 results on TyDi QA zero-shot, we report the median across five fine-tuning runs, as we observed high variance across runs. Full results for all languages in all tasks are provided in the appendix.
}

% Apart from mT5 (ours), XLM-R and \textsc{Filter} metrics are from \citet{fang2020filter}, though \citet{conneau2019unsupervised} report better performance of XLM-R on XNLI (80.9). VECO metrics are from \citet{luo2020veco} and RemBERT from \citet{chung2020rethinking}.
% We compare with baselines from prior work, ignoring leaderboard submissions not described in papers.
\label{tbl:detailed_results_full}
%\vspace{-3mm}
% Acc. is short for Accuracy.
\end{table*}

==> mt5 arxiv 031121/results/mlqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccc|c}
\toprule
Model & en & ar & de & es & hi & vi & zh & avg \\
\midrule
\multicolumn{8}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 80.2 / 67.0 &  52.3 / 34.6 &  59.0 / 43.8 &  67.4 / 49.2 &  50.2 / 35.3 &  61.2 / 40.7 &  59.6 / 38.6 & 61.4 / 44.2\\
XLM & 68.6 / 55.2 &  42.5 / 25.2 &  50.8 / 37.2 &  54.7 / 37.9 &  34.4 / 21.1 &  48.3 / 30.2 &  40.5 / 21.9 & 48.5 / 32.6\\
%MMTE & 78.5 / – &  56.1 / – &  58.4 / – &  64.9 / – &  46.2 / – &  59.4 / – &  58.3 / –  & 60.3 / 41.4\\
XLM-R & 83.5 / 70.6 &  66.6 / 47.1 &  70.1 / 54.9 &  74.1 / 56.6 &  70.6 / 53.1 &  74.0 / 52.9 &  62.1 / 37.0 & 71.6 / 53.2\\
%\textsc{Filter} & 83.5 / 70.3 & 71.8 / 51.0 & 74.6 / 59.8 & 77.9 / 60.2 & 76.1 / 57.7 & 77.7 / 57.2 & 69.0 / 44.2 & 75.8 / 57.2 \\
mT5-Small & 77.2 / 63.0 & 44.7 / 27.3 & 53.3 / 35.7 & 60.1 / 41.5 & 43.0 / 29.2 & 52.9 / 33.2 & 51.3 / 29.7 & 54.6 / 37.1 \\
mT5-Base  & 81.7 / 66.9 & 57.1 / 36.9 & 62.1 / 43.2 & 67.1 / 47.2 & 55.4 / 37.9 & 65.9 / 44.1 & 61.6 / 38.6 & 64.4 / 45.0 \\
mT5-Large & 84.9 / 70.7 & 65.3 / 44.6 & 68.9 / 51.8 & 73.5 / 54.1 & 66.9 / 47.7 & 72.5 / 50.7 & 66.2 / 42.0 & 71.2 / 51.7 \\
mT5-XL    & 85.5 / 71.9 & 68.0 / 47.4 & 70.5 / 54.4 & 75.2 / 56.3 & 70.5 / 51.0 & 74.2 / 52.8 & 70.5 / 47.2 & 73.5 / 54.4 \\
%mT5-XXL (75\%)  & \textbf{86.4} / \textbf{73.0} & \textbf{70.0} / \textbf{49.6} & \textbf{72.8} / \textbf{56.5} & \textbf{76.3} / \textbf{58.2} & \textbf{74.8} / \textbf{56.6} & \textbf{76.4} / \textbf{56.0} & \textbf{72.0} / \textbf{48.8} & \textbf{75.5} / \textbf{56.9} \\
mT5-XXL & \textbf{86.7 / 73.5} & \textbf{70.7 / 50.4} & \textbf{74.0 / 57.8} & \textbf{76.8 / 58.4} & \textbf{75.6 / 57.3} & \textbf{76.4 / 56.0} & \textbf{71.8 / 48.8} & \textbf{76.0 / 57.4}
 \\
\midrule
\multicolumn{8}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%\textsc{Filter} + Self-Teaching & 84.0 / 70.8 & \textbf{72.1} / \textbf{51.1} & \textbf{74.8} /\textbf{60.0} & 78.1 / 60.1 & \textbf{76.0} / \textbf{57.6} & \textbf{78.1} /\textbf{57.5} & 70.5 / 47.0 & 76.2 / 57.7 \\
mT5-Small & 70.5 / 56.2 & 49.3 / 31.0 & 55.6 / 40.6 & 60.5 / 43.0 & 50.4 / 32.9 & 55.2 / 36.3 & 54.4 / 31.6 & 56.6 / 38.8 \\
mT5-Base & 80.7 / 66.3 & 61.1 / 40.7 & 65.5 / 49.2 & 70.7 / 52.1 & 63.6 / 44.3 & 68.0 / 47.6 & 63.5 / 39.4 & 67.6 / 48.5 \\
mT5-Large & 85.3 / 72.0 & 68.5 / 47.7 & 71.6 / 55.8 & 75.7 / 57.1 & 71.8 / 52.6 & 74.3 / 54.0 & 70.1 / 47.1 & 73.9 / 55.2 \\
mT5-XL & 86.0 / 73.0 & 70.0 / 49.8 & 72.7 / 56.8 & 76.9 / 58.3 & 73.4 / 55.0 & 75.4 / 55.0 & 71.4 / 48.4 & 75.1 / 56.6 \\
mT5-XXL & \textbf{86.5 / 73.5} &	\textbf{71.7 / 51.4} &	\textbf{74.9 / 58.7} &	\textbf{78.8 / 60.3} &	\textbf{76.6 / 58.5} &	\textbf{77.1 / 56.3} &	\textbf{72.5 / 49.8} &	\textbf{76.9 / 58.3} \\
\bottomrule
\end{tabular}
\caption{MLQA results (F1/EM) for each language.}
%\vspace{-3mm}
\end{table*}

==> mt5 arxiv 031121/results/ner.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|cccccccccccccccccccc|c}
\toprule
Model & af & ar & bg & bn & de & el & en & es & et & eu & fa & fi & fr & he & hi & hu & id & it & ja & jv & \\
\midrule
\multicolumn{17}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 77.4 & 41.1 & 77.0 & 70.0 & 78.0 & 72.5 & 85.2 & 77.4 & 75.4 & \textbf{66.3} & 46.2 & 77.2 & 79.6 & 56.6 & 65.0 & 76.4 & 53.5 & 81.5 & 29.0 & \textbf{66.4} & \\
XLM & 74.9 & 44.8 & 76.7 & 70.0 & 78.1 & 73.5 & 82.6 & 74.8 & 74.8 & 62.3 & 49.2 & \textbf{79.6} & 78.5 & 57.7 & 66.1 & 76.5 & 53.1 & 80.7 & 23.6 & 63.0 & \\
% Phang et. al & 78.5 & 49.2 & 82.0 & 73.3 & 78.9 & 80.1 & 84.5 & 76.6 & 78.5 & 59.4 & 49.4 & 79.1 & 81.2 & 56.4 & 70.6 & 81.0 & 57.0 & 80.7 & 20.7 & 64.7 & \\
XLM-R & 78.9 & 53.0 & 81.4 & 78.8 & 78.8 & \textbf{79.5} & 84.7 & 79.6 & \textbf{79.1} & 60.9 & \textbf{61.9} & 79.2 & 80.5 & 56.8 & 73.0 & \textbf{79.8} & 53.0 & 81.3 & 23.2 & 62.5 & \\
mT5-Small & 67.4 & 36.6 & 64.6 & 60.4 & 66.1 & 59.1 & 80.7 & 63.6 & 58.4 & 42.3 & 25.3 & 64.5 & 74.6 & 39.6 & 57.9 & 61.5 & 46.7 & 73.4 & 28.8 & 50.6 & \\
mT5-Base & 73.8 & 48.4 & 68.2 & 67.1 & 72.5 & 63.5 & 83.2 & 71.7 & 67.3 & 49.2 & 31.9 & 68.6 & 78.6 & 47.4 & 67.6 & 64.7 & 49.7 & 78.9 & 35.3 & 56.9 & \\
mT5-Large & 74.7 & 55.0 & 60.6 & 64.5 & 75.2 & 68.2 & 84.2 & 74.2 & 67.0 & 48.7 & 51.4 & 66.4 & 82.4 & 55.8 & 69.0 & 67.3 & 51.1 & 80.7 & 43.0 & 57.1 & \\
mT5-XL & 79.8 & 60.2 & 81.0 & 78.1 & 80.6 & 78.3 & 86.3 & 74.7 & 71.8 & 52.2 & 61.5 & 70.1 & 86.2 & \textbf{65.5} & 76.5 & 71.9 & 56.8 & 83.3 & 48.0 & 64.5 & \\
mT5-XXL & \textbf{80.4} & \textbf{66.2} & \textbf{85.1} & \textbf{79.3} & \textbf{81.7} & 79.0 & \textbf{86.7} & \textbf{86.0} & 73.5 & 57.6 & 58.8 & 70.4 & \textbf{86.8} & 65.1 & \textbf{77.8} & 74.2 & \textbf{73.5} & \textbf{85.8} & \textbf{50.7} & \textbf{66.4} & \\
\midrule
& ka & kk & ko & ml & mr & ms & my & nl & pt & ru & sw & ta & te & th & tl & tr & ur & vi & yo & zh & avg \\
\midrule
mBERT & 64.6 & 45.8 & 59.6 & 52.3 & 58.2 & 72.7 & 45.2 & 81.8 & 80.8 & 64.0 & 67.5 & 50.7 & 48.5 & 3.6 & 71.7 & 71.8 & 36.9 & 71.8 & 44.9 & 42.7 & 62.2 \\
XLM & 67.7 & \textbf{57.2} & 26.3 & 59.4 & 62.4 & 69.6 & 47.6 & 81.2 & 77.9 & 63.5 & 68.4 & 53.6 & 49.6 & 0.3 & 78.6 & 71.0 & 43.0 & 70.1 & 26.5 & 32.4 & 61.2 \\
% Phang et. al & 68.6 & 53.2 & 57.8 & 60.8 & 61.0 & 69.3 & 54.2 & 83.8 & 80.8 & 69.4 & 70.6 & 58.9 & 53.7 & 2.2 & 75.2 & 77.2 & 57.7 & 75.6 & 46.1 & 30.4 & 64.7 \\
XLM-R & \textbf{71.6} & 56.2 & \textbf{60.0} & \textbf{67.8} & \textbf{68.1} & 57.1 & \textbf{54.3} & 84.0 & 81.9 & 69.1 & 70.5 & \textbf{59.5} & 55.8 & 1.3 & 73.2 & \textbf{76.1} & 56.4 & 79.4 & 33.6 & 33.1 & 65.4 \\
mT5-Small & 53.2 & 23.4 & 26.6 & 39.4 & 39.4 & 70.0 & 30.1 & 75.4 & 70.8 & 46.5 & 54.8 & 37.5 & 32.6 & 7.2 & 69.4 & 56.0 & 26.4 & 63.8 & 58.8 & 37.9 & 51.0 \\
mT5-Base & 50.1 & 23.4 & 33.9 & 48.2 & 43.8 & 72.6 & 37.0 & 80.1 & 76.0 & 55.4 & 62.4 & 41.2 & 42.7 & 9.5 & 74.6 & 58.4 & 38.4 & 73.0 & 59.3 & 41.5 & 56.6 \\
mT5-Large & 58.2 & 23.3 & 36.2 & 46.3 & 46.5 & 69.4 & 32.2 & 82.7 & 79.6 & 50.2 & 72.4 & 46.4 & 44.5 & \textbf{10.5} & 79.0 & 65.1 & 44.2 & 77.1 & 48.4 & 44.0 & 58.8 \\
mT5-XL & 66.0 & 31.6 & 38.1 & 54.1 & 57.6 & 74.8 & 42.6 & 85.7 & 85.2 & 66.9 & 72.8 & 49.0 & 54.7 & 9.6 & 84.1 & 67.7 & 64.7 & 79.6 & 59.9 & 54.4. & 65.7 \\
mT5-XXL & 66.0 & 38.7 & 43.5 & 54.5 & 63.1 & \textbf{77.6} & 44.7 & \textbf{87.7} & \textbf{86.9} & \textbf{72.0} & \textbf{72.9} & 56.5 & \textbf{59.5} & 10.4 & \textbf{85.2} & 71.4 & \textbf{80.7} & \textbf{84.6} & \textbf{70.0} & \textbf{56.8} & \textbf{69.2} \\
\bottomrule
\end{tabular}
\caption{WikiAnn NER F1 scores for each language.}
\end{table*}

==> mt5 arxiv 031121/results/pawsx.tex <==
\begin{table*}[h!]
\centering
\footnotesize
% Manually specify the width of the last column. Otherwise the last column is too wide.
\begin{tabular}{l|p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}|p{3em}<{\centering\arraybackslash}}
\toprule
Model & en & de & es & fr & ja & ko & zh & avg \\
\midrule
\multicolumn{9}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 94.0& 85.7& 87.4& 87.0& 73.0& 69.6& 77.0 & 81.9 \\
XLM & 94.0& 85.9& 88.3& 87.4& 69.3& 64.8& 76.5 & 80.9 \\
%MMTE & 93.1& 85.1& 87.2& 86.9& 72.0& 69.2& 75.9 & 81.3 \\
XLM-R & 94.7& 89.7& 90.1& 90.4& 78.7& 79.0& 82.3 & 86.4 \\
%\textsc{Filter} & 96.5 & 92.5 & 93.0 & 93.8 & 86.7 & 87.1 & 88.3 & 91.2 \\
mT5-Small           & 92.2 & 86.2 & 86.1 & 86.6 & 74.7 & 73.5 & 77.9 & 82.4 \\
mT5-Base            & 95.4 & 89.4 & 89.6 & 91.2 & 79.8 & 78.5 & 81.1 & 86.4 \\
mT5-Large           & 96.1 & 91.3 & 92.0   & \textbf{92.7} & 82.5 & 82.7 & 84.7 & 88.9 \\
mT5-XL              & 96.0   & 92.8 & \textbf{92.7} & 92.4 & 83.6 & 83.1 & 86.5 & 89.6 \\
%mT5-XXL (75\%)      & 95.7 & 91.6 & 91.6 & 92.3 & 83.4 & 82.9 & \textbf{86.8} & 89.2 \\
mT5-XXL & \textbf{96.3} & \textbf{92.9} & 92.6 & \textbf{92.7} & \textbf{84.5} & \textbf{83.9} & \textbf{87.2} & \textbf{90.0} \\
\midrule
\multicolumn{9}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%\textsc{Filter} + Self-Teaching & 95.9 & 92.8 & 93.0 & 93.7 & \textbf{87.4} & 87.6 & 89.6 & 91.4 \\
mT5-Small & 87.9 & 81.4 & 83.1 & 84.1 & 74.2 & 71.7 & 76.7 & 79.9 \\
mT5-Base & 95.5 & 90.9 & 91.4 & 92.5 & 83.6 & 84.8 & 86.4 & 89.3 \\
mT5-Large & 96.4 & 92.7 & 93.3 & 93.6 & 86.5 & 87.4 & 88.4 & 91.2 \\
mT5-XL & 96.4 & 92.5 & 93.1 & 93.6 & 85.5 & 86.9 & \textbf{89.0} & 91.0 \\
mT5-XXL & \textbf{96.1} & \textbf{92.9} & \textbf{93.6} & \textbf{94.2} & \textbf{87.0} & \textbf{87.9} & \textbf{89.0} & \textbf{91.5} \\
\bottomrule
\end{tabular}
\caption{PAWS-X accuracy scores for each language.}
%\vspace{-3mm}
\end{table*}

==> mt5 arxiv 031121/results/tydiqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccc|c}
\toprule
Model &  en & ar & bn & fi & id & ko & ru & sw & te & avg \\

\midrule
\multicolumn{8}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule

mBERT & 75.3 / 63.6 &  62.2 / 42.8 &  49.3 / 32.7 &  59.7 / 45.3 &  64.8 / 45.8 &  58.8 / 50.0 &  60.0 / 38.8 &  57.5 / 37.9 &  49.6 / 38.4 &  59.7 / 43.9 \\
XLM & 66.9 / 53.9 &  59.4 / 41.2 &  27.2 / 15.0 &  58.2 / 41.4 &  62.5 / 45.8 &  14.2 / 5.1 &  49.2 / 30.7 &  39.4 / 21.6 &  15.5 / 6.9 &  43.6 / 29.1 \\
%MMTE & 62.9 / 49.8 &  63.1 / 39.2 &  55.8 / 41.9 &  53.9 / 42.1 &  60.9 / 47.6 &  49.9 / 42.6 &  58.9 / 37.9 &  63.1 / 47.2 &  54.2 / 45.8 &  58.1 / 43.8 \\
XLM-R & 71.5 / 56.8 &  67.6 / 40.4 &  64.0 / 47.8 &  70.5 / 53.2 &  77.4 / 61.9 &  31.9 / 10.9 &  67.0 / 42.1 &  66.1 / 48.1 &  70.1 / 43.6 &  65.1 / 45.0 \\
%\textsc{Filter} & 71.9 / 58.9 & 73.7 / 47.9 & 68.7 / 53.1 & 71.2 / 54.9 & 77.9 / 59.8 & 33.0 / 12.3 & 68.7 / 45.9 & 78.7 / 66.1 & 69.4 / 48.6 & 68.1 / 49.7 \\
mT5-Small & 53.9 / 43.6 & 41.1 / 26.0 & 18.9 / 13.3 & 39.2 / 22.6 & 44.4 / 31.7 & 24.9 / 16.3 & 40.5 / 24.3 & 34.8 / 21.2 & 16.9 / 11.5 & 34.9 / 23.4 \\
mT5-Base & 71.8 / 60.9 & 67.1 / 50.4 & 40.7 / 22.1 & 67.0 / 52.2 & 71.3 / 54.5 & 49.5 / 37.7 & 54.9 / 32.6 & 60.4 / 43.9 & 40.6 / 31.1 & 58.1 / 42.8 \\
mT5-Large & 71.6 / 58.9 & 60.5 / 40.4 & 42.0 / 23.9 & 64.6 / 48.8 & 67.0 / 49.2 & 47.6 / 37.3 & 58.9 / 36.8 & 65.7 / 45.3 & 41.9 / 29.7 & 57.8 / 41.2 \\
mT5-XL & 80.3 / 70.9 & 81.7 / 65.5 & 74.5 / 57.5 & 79.4 / 65.3 & 83.5 / 70.4 & 70.0 / 60.5 & 71.6 / 47.8 & 77.3 / 59.7 & 77.9 / 55.8 & 77.4 / 61.5 \\
%mT5-XXL (75\%) & \textbf{83.1} / \textbf{72.3}	& \textbf{83.3} / \textbf{67.2}	&	\textbf{80.9} / \textbf{68.1}	&	\textbf{82.9} / \textbf{70.2}	&	\textbf{86.3} / \textbf{75.6}	&	\textbf{73.7} / \textbf{63.0}	&	\textbf{75.2} / \textbf{53.8}	&	\textbf{82.4} / \textbf{66.5}	&	\textbf{79.2} / \textbf{59.6}	&	\textbf{80.8} / \textbf{66.3} \\
mT5-XXL & \textbf{83.7 / 72.5} & \textbf{82.8 / 66.0} & \textbf{80.2 / 63.7} & \textbf{83.3 / 70.2} & \textbf{85.3 / 73.3} & \textbf{76.2 / 64.1} & \textbf{76.6 / 55.8} & \textbf{81.9 / 66.1} & \textbf{79.2 / 58.7} & \textbf{81.0 / 65.6} \\

\midrule
\multicolumn{8}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule

%\textsc{Filter} + Self-Teaching & 72.4 / 59.1 & 72.8 / 50.8 & 70.5 / 56.6 & 73.3 / 57.2 & 76.8 / 59.8 & 33.1 / 12.3 & 68.9 / 46.6 & 77.4 / 65.7 & 69.9 / 50.4 & 68.3 / 50.9 \\
mT5-Small & 57.1 / 46.6 & 56.8 / 39.7 & 37.2 / 21.2 & 50.9 / 37.2 & 60.1 / 45.1 & 40.4 / 29.3 & 50.7 / 33.6 & 51.5 / 35.3 & 29.3 / 18.1 & 48.2 / 34.0 \\
mT5-Base & 71.1 / 58.9 & 68.0 / 50.2 & 57.4 / 35.4 & 68.8 / 55.2 & 73.5 / 57.2 & 56.5 / 43.8 & 64.0 / 45.8 & 65.8 / 48.3 & 51.2 / 34.1 & 64.0 / 47.7 \\
mT5-Large & 75.6 / 62.7 & 74.8 / 57.9 & 65.0 / 46.0 & 72.3 / 57.5 & 78.7 / 63.5 & 66.4 / 53.6 & 70.9 / 50.5 & 74.0 / 56.7 & 62.0 / 45.1 & 71.1 / 54.9 \\
mT5-XL & 82.0 / 65.7 &	79.3 / 65.5 &	80.4 / 68.9 &	79.1 / 64.7 &	84.7 / 71.0 &	70.5 / 56.2 &	78.3 / 61.1 &	83.9 / 70.9 &	80.9 / 64.0 &	79.9 / 65.3 \\
mT5-XXL & \textbf{83.3 / 71.6} & \textbf{83.0 / 66.3} & \textbf{82.3 / 70.8} & \textbf{82.9 / 67.8} & \textbf{86.6 / 72.0} & \textbf{75.0 / 62.3} & \textbf{80.7 / 63.1} & \textbf{86.9 / 75.8} & \textbf{84.6 / 69.2} & \textbf{82.8 / 68.8} \\

\midrule
\multicolumn{8}{l}{\emph{In-language multitask (models fine-tuned on gold data in all target languages)}} \\
\midrule

mT5-Small & 66.4 / 56.1	& 80.3 / 68.7 & 71.7 / 60.2 & 71.9 / 59.5 & 78.8 / 67.6 & 55.5 / 46.7 & 70.1 / 57.1 & 77.7 / 68.9 & 82.7 / 71.6 & 73.0 / 62.0 \\
mT5-Base & 76.6 / 65.2 & 84.2 / 71.8 & 80.0 / 69.0 & 80.1 / 69.3 & 85.5 / 75.0 & 70.3 / 61.6 & 77.5 / 64.4 & 83.6 / 74.9 & 88.2 / 78.0 & 80.8 / 70.0 \\
mT5-Large & 82.4 / 70.9 & 87.1 / 75.1 & 86.3 / 78.8 & 85.5 / 73.4 & 87.3 / 77.9 & 79.1 / 69.9 & 84.3 / 71.3 & 87.4 / 79.6 & 90.2 / 81.2 & 85.5 / 75.3 \\
mT5-XL & 84.1 / 74.3 & \textbf{88.5} / 76.0 & 87.7 / \textbf{80.5} & 87.4 / 76.1 & 89.9 / 81.2 & 82.8 / 75.4 & 84.9 / 73.2 & 90.1 / 82.8 & 92.0 / 83.7 & 87.5 / 78.1 \\
mT5-XXL & \textbf{85.7 / 75.5} & 88.4 / \textbf{76.9} & \textbf{88.7 / 80.5} & \textbf{87.5 / 76.3} & \textbf{90.3 / 81.8} & \textbf{83.7 / 75.7} & \textbf{87.9 / 76.8} & \textbf{91.9 / 84.4} & \textbf{92.6 / 83.9} & \textbf{88.5 / 79.1} \\

\bottomrule
\end{tabular}
\caption{TyDi QA GoldP results (F1/EM) for each language.}
%\vspace{-3mm}
\end{table*}





==> mt5 arxiv 031121/results/xnli.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccccccc|c}
\toprule
Model & en & ar & bg & de & el & es & fr & hi & ru & sw & th & tr & ur & vi & zh & avg \\
\midrule
\multicolumn{17}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule

mBERT &80.8& 64.3& 68.0& 70.0& 65.3& 73.5& 73.4& 58.9& 67.8& 49.7& 54.1& 60.9& 57.2& 69.3& 67.8& 65.4 \\
XLM &82.8& 66.0& 71.9& 72.7& 70.4& 75.5& 74.3& 62.5& 69.9& 58.1& 65.5& 66.4& 59.8& 70.7& 70.2& 69.1 \\
XLM-R &88.7& 77.2& 83.0& 82.5& 80.8& 83.7& 82.2& 75.6& 79.1& 71.2& 77.4& 78.0& 71.7& 79.3& 78.2& 79.2 \\
mT5-Small & 79.6 & 65.2 & 71.3 & 69.2 & 68.6  & 72.7 & 70.7 & 62.5 & 70.1 & 59.7 & 66.3 & 64.4 & 59.9 & 66.3 & 65.8 & 67.5 \\
mT5-Base & 84.7 & 73.3 & 78.6 & 77.4 & 77.1  & 80.3 & 79.1 & 70.8 & 77.1 & 69.4 & 73.2 & 72.8 & 68.3 & 74.2 & 74.1 & 75.4 \\
mT5-Large & 89.4 & 79.8 & 84.1 & 83.4 & 83.2  & 84.2 & 84.1 & 77.6 & 81.5 & 75.4 & 79.4 & 80.1 & 73.5 & 81.0 & 80.3 & 81.1 \\
mT5-XL & 90.6 & 82.2 & 85.4 & 85.8 & 85.4  & 81.3 & 85.3 & 80.4 & 83.7 & 78.6 & 80.9 & 82.0 & 77.0 & 81.8 & 82.7 & 82.9 \\
%mT5-XXL (75\%) & \textbf{92.3} & \textbf{84.4}& \textbf{87.5}& \textbf{87.3}& \textbf{87.0}&  \textbf{88.3}& \textbf{87.3}& \textbf{82.5}& \textbf{84.3}& \textbf{80.4}& \textbf{81.7}& \textbf{83.3}& \textbf{79.2}& \textbf{84.2}& \textbf{82.7}& \textbf{84.8}\\
mT5-XXL & \textbf{91.6} & \textbf{84.5} & \textbf{87.7} & \textbf{87.3} & \textbf{87.3} & \textbf{87.8} & \textbf{86.9} & \textbf{83.2} & \textbf{85.1} & \textbf{80.3} & \textbf{81.7} & \textbf{83.8} & \textbf{79.8} & \textbf{84.6} & \textbf{83.6} & \textbf{84.5} \\
\midrule
\multicolumn{17}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%Filter + Self-Teaching & 89.5 & 83.6 & 86.4 & 85.6 & 85.4 & 86.6 & 85.7 & 81.1 & 83.7 & 78.7 & 81.7 & 83.2 & 79.1 & 83.9 & 83.8 & 83.9 \\
mt5-Small & 69.5 & 63.7 & 67.5 & 65.7 & 66.4 & 67.5 & 67.3 & 61.9 & 66.4 & 59.6 & 63.9 & 63.5 & 60.4 & 63.3 & 64.5 & 64.7 \\
mt5-Base & 82.0 & 74.4 & 78.5 & 77.7 & 78.1 & 79.1 & 77.9 & 72.2 & 76.5 & 71.5 & 75.0 & 74.8 & 70.4 & 74.5 & 76.0 & 75.9 \\
mt5-Large & 88.3 & 80.3 & 84.1 & 84.0 & 83.7 & 84.9 & 83.8 & 79.8 & 82.0 & 76.4 & 79.9 & 81.0 & 75.9 & 81.3 & 81.7 & 81.8 \\
mt5-XL & 90.9 & 84.2 & 86.8 & 86.8 & 86.4 & 87.4 & 86.8 & 83.1 & 84.9 & 81.3 & 82.3 & 84.4 & 79.4 & 83.9 & 84.0 & 84.8 \\
mT5-XXL & \textbf{92.7} & \textbf{87.2} & \textbf{89.4} & \textbf{89.8} & \textbf{89.5} & \textbf{90.0} & \textbf{89.1} & \textbf{86.5} & \textbf{87.6} & \textbf{84.3} & \textbf{85.6} & \textbf{87.1} & \textbf{83.8} & \textbf{87.5} & \textbf{86.5} & \textbf{87.8} \\
\bottomrule
\end{tabular}
\caption{XNLI accuracy scores for each language.}
\end{table*}

==> mt5 arxiv 031121/results/xnli_ablation.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccccccc|c}
\toprule
Model & ar & bg & de & el & en & es & fr & hi & ru & sw & th & tr & ur & vi & zh & avg \\
\midrule
Baseline (mT5-large) & \textbf{79.8} & \textbf{84.1} & 83.4 & \textbf{83.2} & \textbf{89.4} & 84.2 & 84.1 & \textbf{77.6} & 81.5 & \textbf{75.4} & \textbf{79.4} & \textbf{80.1} & 73.5 & \textbf{81.0} & \textbf{80.3} & \textbf{81.1} \\
Dropout $0.1$ & 76.4 & 82.1 & 81.7 & 81.0 & 88.0 & 70.8 & 80.3 & 74.4 & 79.0 & 72.3 & 75.8 & 75.9 & 70.6 & 78.6 & 76.5 & 77.6 \\
Sequence length $512$ & 78.1 & 83.4 & 83.1 & 82.1 & 88.8 & 84.5 & 82.8 & 77.3 & 81.2 & \textbf{75.4} & 78.2 & 79.6 & 73.8 & 80.0 & 78.9 & 80.5 \\
Span length $10$ & 77.6 & 81.5 & 80.5 & 81.2 & 87.2 & 83.0 & 81.2 & 74.7 & 79.8 & 73.6 & 76.7 & 75.9 & 71.3 & 78.6 & 76.5 & 78.6 \\
$\alpha = 0.7$ & 79.3 & \textbf{84.1} & \textbf{84.5} & 83.1 & \textbf{89.4} & \textbf{85.3} & \textbf{84.4} & 76.4 & \textbf{82.8} & 70.6 & 78.7 & 79.8 & 71.7 & 80.3 & 79.9 & 80.7 \\
$\alpha = 0.2$ & 78.7 &83.8 &83.3 &82.5 &89.3 &83.4 &83.6 &77.3 &81.2 &\textbf{75.4} &78.6 &79.4 &\textbf{73.9} &79.9 &79.7 &80.7 \\
No line length filter & 78.4 & 83.3 & 81.5 & 81.4 & 88.9 & 83.8 & 82.5 & 74.4 & 80.5 & 69.4 & 77.6 & 76.9 & 71.3 & 78.8 & 78.3 & 79.1 \\
Add Wikipedia data & 79.3& 83.1& 83.1& 82.7& 88.6& 80.1& 83.2& 77.3& 81.4& 75.0& 78.9& 79.3& 73.5& 80.2& 79.2& 80.3\\
% Finetune 2M steps &79.7& 84.3& 83.7& 83.3& 89.3& 85.1& 84.1& 77.5& 81.9& 75.5& 79.1& 79.4& 74.3& 81.5& 79.6& 81.2 \\
% Train 2M dropout & 73.4& 79.0& 79.3& 77.7& 86.0& 62.5& 72.4& 71.6& 76.1& 69.1& 72.6& 68.9& 67.2& 75.1& 73.8& 73.7 \\
\bottomrule
\end{tabular}
\caption{XNLI zero-shot accuracy of various ablations on our mT5-Large model.}
\end{table*}

==> mt5 arxiv 031121/results/xquad.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccc|c}
\toprule
Model & en & ar & de & el & es & hi & ru & th & tr & vi & zh & avg \\
\midrule
\multicolumn{8}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 83.5 / 72.2 &  61.5 / 45.1 &  70.6 / 54.0 &  62.6 / 44.9 &  75.5 / 56.9 &  59.2 / 46.0 &  71.3 / 53.3 &  42.7 / 33.5 &  55.4 / 40.1 &  69.5 / 49.6 &  58.0 / 48.3 &  64.5 / 49.4 \\
XLM & 74.2 / 62.1 &  61.4 / 44.7 &  66.0 / 49.7 &  57.5 / 39.1 &  68.2 / 49.8 &  56.6 / 40.3 &  65.3 / 48.2 &  35.4 / 24.5 &  57.9 / 41.2 &  65.8 / 47.6 &  49.7 / 39.7 &  59.8 / 44.3 \\
%MMTE & 80.1 / 68.1 &  63.2 / 46.2 &  68.8 / 50.3 &  61.3 / 35.9 &  72.4 / 52.5 &  61.3 / 47.2 &  68.4 / 45.2 &  48.4 / 35.9 &  58.1 / 40.9 &  70.9 / 50.1 &  55.8 / 36.4 &  64.4 / 46.2 \\
XLM-R & 86.5 / 75.7 &  68.6 / 49.0 &  80.4 / 63.4 &  79.8 / 61.7 &  82.0 / 63.9 &  76.7 / 59.7 &  \textbf{80.1 / 64.3} &  74.2 / 62.8
&  75.9 / 59.3 &  79.1 / 59.0 &  59.3 / 50.0 &  76.6 / 60.8 \\
%\textsc{Filter} & 85.6 / 73.0 & 79.8 / 61.3 & 82.5 / 66.2 & 82.6 / 64.6 & 84.8 / 67.4 & 83.1 / 66.5 & 82.5 / 66.8 & 80.7 / 73.9 & 81.2 / 65.7 & 83.3 / 64.1 & 78.9 / 75.7 & 82.3 / 67.8 \\
mT5-Small & 78.5 / 66.1 & 51.4 / 34.0 & 63.8 / 45.9 & 53.8 / 33.4 & 67.0 / 50.3 & 47.8 / 34.5 & 50.5 / 30.1 & 54.0 / 44.5 & 55.7 / 38.9 & 58.1 / 41.3 & 58.9 / 48.7 & 58.1 / 42.5 \\
mT5-Base & 84.6 / 71.7 & 63.8 / 44.3 & 73.8 / 54.5 & 59.6 / 35.6 & 74.8 / 56.1 & 60.3 / 43.4 & 57.8 / 34.7 & 57.6 / 45.7 & 67.9 / 48.2 & 70.7 / 50.3 & 66.1 / 54.1 & 67.0 / 49.0 \\
mT5-Large & 88.4 / 77.3 & 75.2 / 56.7 & 80.0 / 62.9 & 77.5 / 57.6 & 81.8 / 64.2 & 73.4 / 56.6 & 74.7 / 56.9 & 73.4 / 62.0 & 76.5 / 56.3 & 79.4 / 60.3 & 75.9 / 65.5 & 77.8 / 61.5 \\
mT5-XL & 88.8 / 78.1 & 77.4 / 60.8 & 80.4 / 63.5 & 80.4 / 61.2 & 82.7 / 64.5 & 76.1 / 60.3 & 76.2 / 58.8 & 74.2 / 62.5 & 77.7 / 58.4 & 80.5 / 60.8 & 80.5 / 71.0 & 79.5 / 63.6 \\
%mT5-XXL (75\%) & \textbf{90.8} / \textbf{79.7} & \textbf{79.7} / \textbf{62.7} & \textbf{83.6} / \textbf{66.8} & \textbf{82.0} / \textbf{64.0} & \textbf{84.7} / \textbf{67.9} & \textbf{81.0} / \textbf{64.8} & \textbf{80.2} / 64.0 & 72.9 / 58.1 & \textbf{80.0} / \textbf{59.9} & \textbf{83.0} / \textbf{62.9} & \textbf{82.5} / \textbf{71.6} & \textbf{81.9} / \textbf{65.7} \\
mT5-XXL & \textbf{90.9 / 80.1} & \textbf{80.3 / 62.6} & \textbf{83.1 / 65.5} & \textbf{83.3 / 65.5} & \textbf{85.1 / 68.1} & \textbf{81.7 / 65.9} & 79.3 / 63.6 & \textbf{77.8 / 66.1} & \textbf{80.2 / 60.9} & \textbf{83.1 / 63.6} & \textbf{83.1 / 73.4} & \textbf{82.5 / 66.8}
 \\
\midrule
\multicolumn{8}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%\textsc{Filter} + Self-Teaching & 86.4 / 74.6 & 79.5 / 60.7 & 83.2 / 67.0 & 83.0 / 64.6 & 85.0 / 67.9 & 83.1 / 66.6 & 82.8 / 67.4 & \textbf{79.6} / \textbf{73.2} & 80.4 / 64.4 & 83.8 / 64.7 & 79.9 / 77.0 & 82.4 / 68.0 \\
mT5-Small & 74.0 / 61.2 & 61.0 / 45.0 & 66.0 / 50.2 & 64.1 / 47.2 & 67.5 / 50.8 & 60.2 / 43.7 & 64.4 / 46.7 & 58.9 / 52.9 & 59.0 / 39.4 & 63.5 / 46.0 & 68.2 / 61.2 & 64.3 / 49.5 \\
mT5-Base & 83.1 / 70.3 & 72.4 / 55.2 & 76.9 / 59.7 & 76.8 / 58.8 & 79.0 / 61.2 & 71.4 / 53.4 & 76.1 / 58.5 & 67.9 / 62.0 & 72.5 / 51.4 & 75.9 / 56.3 & 76.9 / 69.7 & 75.3 / 59.7 \\
mT5-Large & 87.3 / 75.5 & 79.4 / 62.7 & 82.7 / 66.0 & 81.8 / 63.5 & 83.8 / 66.1 & 78.0 / 59.8 & 81.9 / 66.3 & 74.7 / 68.2 & 80.2 / 59.2 & 80.4 / 60.8 & 83.2 / 76.9 & 81.2 / 65.9 \\
mT5-XL & 88.5 / 77.1 & 80.9 / 65.4 & 83.4 / 66.7 & 83.6 / 64.9 & 84.9 / 68.2 & 79.6 / 63.1 & 82.7 / 67.1 & 78.5 / 72.9 & 82.4 / 63.8 & 82.4 / 64.1 & 83.2 / 75.9 & 82.7 / 68.1 \\
mT5-XXL & \textbf{91.3 / 80.3} &	\textbf{83.4 / 68.2} &	\textbf{85.0 / 68.2} &	\textbf{85.9 / 68.9} &	\textbf{87.4 / 70.8} &	\textbf{83.7 / 68.2} &	\textbf{85.2 / 70.4} &	\textbf{80.2 / 74.5} &	\textbf{84.4 / 67.7} &	\textbf{85.3 / 67.1} &	\textbf{85.7 / 80.0} &	\textbf{85.2 / 71.3} \\
\bottomrule
\end{tabular}
\caption{XQuAD results (F1/EM) for each language.}
%\vspace{-3mm}
\end{table*}

==> mt5 arxiv 031121/results/xquad_ablation.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccc|c}
\toprule   
Model & en & ar & de & el & es & hi & ru & th & tr & vi & zh & avg \\
\midrule
Baseline(mT5-large) & 88.4 / 77.3    & 75.2 / 56.7    & 80.0 / \textbf{62.9}    & 77.5 / 57.6    & \textbf{81.8} / 64.2    & 73.4 / 56.6    & 74.7 / 56.9    & 73.4 / \textbf{62.0}    & 76.5 / 56.3    & 79.4 / \textbf{60.3}    & 75.9 / 65.5 & 77.8 / 61.5 \\
Span length $10$   & 88.1 / 76.3   & 70.0 / 50.6   & 78.1 / 60.2   & 68.8 / 44.0   & 79.0 / 60.8   & 67.3 / 48.4   & 65.4 / 43.3   & 68.1 / 57.2   & 74.4 / 53.6   & 77.9 / 57.7   & 76.6 / 66.4   & 74.0 / 56.2   \\
Dropout $0.1$   & 87.3 / 76.0   & 54.9 / 33.9   & 77.6 / 60.2   & 64.4 / 40.1   & 79.2 / 60.6   & 59.1 / 40.4   & 59.5 / 38.4   & 65.7 / 51.0   & 73.6 / 52.8   & 75.8 / 55.8   & 77.0 / 64.5   & 70.4 / 52.1   \\
Sequence length $512$  & 88.0 / 76.9   & \textbf{77.0} / 59.6   & 80.2 / 62.4   & \textbf{79.8} / \textbf{60.0}   & 81.7 / \textbf{64.4}   & \textbf{75.1} / \textbf{57.5}   & \textbf{77.4} / \textbf{58.5}   & 72.7 / 59.8   & 75.3 / 53.9   & 79.4 / 58.9   & 78.5 / 67.2   & \textbf{78.6} / \textbf{61.7}   \\
$\alpha = 0.7$  & 88.4 / 77.1   & 76.5 / 58.8   & 78.5 / 59.8   & 77.2 / 55.5   & 78.7 / 59.5   & 74.6 / 56.8   & 73.1 / 54.5   & 72.5 / 60.2   & 75.7 / 55.0   & 79.2 / 58.3   & \textbf{78.6} / 66.2   & 77.5 / 60.2   \\
 $\alpha = 0.2$  & 87.9 / 76.8   & 75.5 / 57.3   & 80.2 / 62.4   & 76.2 / 54.0   & 81.6 / 63.7   & 73.7 / 57.0   & 70.7 / 50.8   & 72.2 / 60.4   & 75.5 / 55.7   & \textbf{79.7} / 59.7   & 78.3 / \textbf{67.5}   & 77.4 / 60.5   \\
No line length filter & 88.9 / 77.4   & 73.8 / 54.0   & \textbf{80.8} / 62.7   & 74.2 / 51.8   & 80.9 / 62.8   & 74.1 / 56.6   & 75.0 / 56.4   & 71.7 / 60.3   & \textbf{76.7} / 56.0   & 78.8 / 58.6   & 78.5 / 67.1   & 77.6 / 60.3   \\
 Add Wikipedia data    & \textbf{89.3} / \textbf{78.4}   & 69.6 / 48.9   & 79.6 / 61.1   & 59.5 / 36.0   & 80.6 / 61.0   & 73.6 / 55.0   & 68.7 / 47.0   & 70.5 / 58.1   & \textbf{76.7} / \textbf{56.9}   & 78.6 / 56.4   & 77.5 / 66.3   & 74.9 / 56.8   \\
% Finetune 2M steps       & 37.5 / 22.7   & 75.7 / \textbf{63.9}   & 58.0 / 38.8   & 58.9 / 42.2   & 62.6 / 45.9   & 32.3 / 21.3   & 31.2 / 17.4   & 60.2 / 50.5   & 50.2 / 33.1   & 58.1 / 39.7   & 39.5 / 31.6   & 51.3 / 37.0  \\

\bottomrule
\end{tabular}
\caption{XQuAD zero-shot F1/EM of various ablations on our mT5-Large model.}
\end{table*}

==> results/mlqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccc|c}
\toprule
Model & en & ar & de & es & hi & vi & zh & avg \\
\midrule
\multicolumn{8}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 80.2 / 67.0 &  52.3 / 34.6 &  59.0 / 43.8 &  67.4 / 49.2 &  50.2 / 35.3 &  61.2 / 40.7 &  59.6 / 38.6 & 61.4 / 44.2\\
XLM & 68.6 / 55.2 &  42.5 / 25.2 &  50.8 / 37.2 &  54.7 / 37.9 &  34.4 / 21.1 &  48.3 / 30.2 &  40.5 / 21.9 & 48.5 / 32.6\\
%MMTE & 78.5 / – &  56.1 / – &  58.4 / – &  64.9 / – &  46.2 / – &  59.4 / – &  58.3 / –  & 60.3 / 41.4\\
XLM-R & 83.5 / 70.6 &  66.6 / 47.1 &  70.1 / 54.9 &  74.1 / 56.6 &  70.6 / 53.1 &  74.0 / 52.9 &  62.1 / 37.0 & 71.6 / 53.2\\
%\textsc{Filter} & 83.5 / 70.3 & 71.8 / 51.0 & 74.6 / 59.8 & 77.9 / 60.2 & 76.1 / 57.7 & 77.7 / 57.2 & 69.0 / 44.2 & 75.8 / 57.2 \\
mT5-Small & 77.2 / 63.0 & 44.7 / 27.3 & 53.3 / 35.7 & 60.1 / 41.5 & 43.0 / 29.2 & 52.9 / 33.2 & 51.3 / 29.7 & 54.6 / 37.1 \\
mT5-Base  & 81.7 / 66.9 & 57.1 / 36.9 & 62.1 / 43.2 & 67.1 / 47.2 & 55.4 / 37.9 & 65.9 / 44.1 & 61.6 / 38.6 & 64.4 / 45.0 \\
mT5-Large & 84.9 / 70.7 & 65.3 / 44.6 & 68.9 / 51.8 & 73.5 / 54.1 & 66.9 / 47.7 & 72.5 / 50.7 & 66.2 / 42.0 & 71.2 / 51.7 \\
mT5-XL    & 85.5 / 71.9 & 68.0 / 47.4 & 70.5 / 54.4 & 75.2 / 56.3 & 70.5 / 51.0 & 74.2 / 52.8 & 70.5 / 47.2 & 73.5 / 54.4 \\
%mT5-XXL (75\%)  & \textbf{86.4} / \textbf{73.0} & \textbf{70.0} / \textbf{49.6} & \textbf{72.8} / \textbf{56.5} & \textbf{76.3} / \textbf{58.2} & \textbf{74.8} / \textbf{56.6} & \textbf{76.4} / \textbf{56.0} & \textbf{72.0} / \textbf{48.8} & \textbf{75.5} / \textbf{56.9} \\
mT5-XXL & \textbf{86.7 / 73.5} & \textbf{70.7 / 50.4} & \textbf{74.0 / 57.8} & \textbf{76.8 / 58.4} & \textbf{75.6 / 57.3} & \textbf{76.4 / 56.0} & \textbf{71.8 / 48.8} & \textbf{76.0 / 57.4}
 \\
\midrule
\multicolumn{8}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%\textsc{Filter} + Self-Teaching & 84.0 / 70.8 & \textbf{72.1} / \textbf{51.1} & \textbf{74.8} /\textbf{60.0} & 78.1 / 60.1 & \textbf{76.0} / \textbf{57.6} & \textbf{78.1} /\textbf{57.5} & 70.5 / 47.0 & 76.2 / 57.7 \\
mT5-Small & 70.5 / 56.2 & 49.3 / 31.0 & 55.6 / 40.6 & 60.5 / 43.0 & 50.4 / 32.9 & 55.2 / 36.3 & 54.4 / 31.6 & 56.6 / 38.8 \\
mT5-Base & 80.7 / 66.3 & 61.1 / 40.7 & 65.5 / 49.2 & 70.7 / 52.1 & 63.6 / 44.3 & 68.0 / 47.6 & 63.5 / 39.4 & 67.6 / 48.5 \\
mT5-Large & 85.3 / 72.0 & 68.5 / 47.7 & 71.6 / 55.8 & 75.7 / 57.1 & 71.8 / 52.6 & 74.3 / 54.0 & 70.1 / 47.1 & 73.9 / 55.2 \\
mT5-XL & 86.0 / 73.0 & 70.0 / 49.8 & 72.7 / 56.8 & 76.9 / 58.3 & 73.4 / 55.0 & 75.4 / 55.0 & 71.4 / 48.4 & 75.1 / 56.6 \\
mT5-XXL & \textbf{86.5 / 73.5} &	\textbf{71.7 / 51.4} &	\textbf{74.9 / 58.7} &	\textbf{78.8 / 60.3} &	\textbf{76.6 / 58.5} &	\textbf{77.1 / 56.3} &	\textbf{72.5 / 49.8} &	\textbf{76.9 / 58.3} \\
\bottomrule
\end{tabular}
\caption{MLQA results (F1/EM) for each language.}
%\vspace{-3mm}
\end{table*}

==> results/ner.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|cccccccccccccccccccc|c}
\toprule
Model & af & ar & bg & bn & de & el & en & es & et & eu & fa & fi & fr & he & hi & hu & id & it & ja & jv & \\
\midrule
\multicolumn{17}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 77.4 & 41.1 & 77.0 & 70.0 & 78.0 & 72.5 & 85.2 & 77.4 & 75.4 & \textbf{66.3} & 46.2 & 77.2 & 79.6 & 56.6 & 65.0 & 76.4 & 53.5 & 81.5 & 29.0 & \textbf{66.4} & \\
XLM & 74.9 & 44.8 & 76.7 & 70.0 & 78.1 & 73.5 & 82.6 & 74.8 & 74.8 & 62.3 & 49.2 & \textbf{79.6} & 78.5 & 57.7 & 66.1 & 76.5 & 53.1 & 80.7 & 23.6 & 63.0 & \\
% Phang et. al & 78.5 & 49.2 & 82.0 & 73.3 & 78.9 & 80.1 & 84.5 & 76.6 & 78.5 & 59.4 & 49.4 & 79.1 & 81.2 & 56.4 & 70.6 & 81.0 & 57.0 & 80.7 & 20.7 & 64.7 & \\
XLM-R & 78.9 & 53.0 & 81.4 & 78.8 & 78.8 & \textbf{79.5} & 84.7 & 79.6 & \textbf{79.1} & 60.9 & \textbf{61.9} & 79.2 & 80.5 & 56.8 & 73.0 & \textbf{79.8} & 53.0 & 81.3 & 23.2 & 62.5 & \\
mT5-Small & 67.4 & 36.6 & 64.6 & 60.4 & 66.1 & 59.1 & 80.7 & 63.6 & 58.4 & 42.3 & 25.3 & 64.5 & 74.6 & 39.6 & 57.9 & 61.5 & 46.7 & 73.4 & 28.8 & 50.6 & \\
mT5-Base & 73.8 & 48.4 & 68.2 & 67.1 & 72.5 & 63.5 & 83.2 & 71.7 & 67.3 & 49.2 & 31.9 & 68.6 & 78.6 & 47.4 & 67.6 & 64.7 & 49.7 & 78.9 & 35.3 & 56.9 & \\
mT5-Large & 74.7 & 55.0 & 60.6 & 64.5 & 75.2 & 68.2 & 84.2 & 74.2 & 67.0 & 48.7 & 51.4 & 66.4 & 82.4 & 55.8 & 69.0 & 67.3 & 51.1 & 80.7 & 43.0 & 57.1 & \\
mT5-XL & 79.8 & 60.2 & 81.0 & 78.1 & 80.6 & 78.3 & 86.3 & 74.7 & 71.8 & 52.2 & 61.5 & 70.1 & 86.2 & \textbf{65.5} & 76.5 & 71.9 & 56.8 & 83.3 & 48.0 & 64.5 & \\
mT5-XXL & \textbf{80.4} & \textbf{66.2} & \textbf{85.1} & \textbf{79.3} & \textbf{81.7} & 79.0 & \textbf{86.7} & \textbf{86.0} & 73.5 & 57.6 & 58.8 & 70.4 & \textbf{86.8} & 65.1 & \textbf{77.8} & 74.2 & \textbf{73.5} & \textbf{85.8} & \textbf{50.7} & \textbf{66.4} & \\
\midrule
& ka & kk & ko & ml & mr & ms & my & nl & pt & ru & sw & ta & te & th & tl & tr & ur & vi & yo & zh & avg \\
\midrule
mBERT & 64.6 & 45.8 & 59.6 & 52.3 & 58.2 & 72.7 & 45.2 & 81.8 & 80.8 & 64.0 & 67.5 & 50.7 & 48.5 & 3.6 & 71.7 & 71.8 & 36.9 & 71.8 & 44.9 & 42.7 & 62.2 \\
XLM & 67.7 & \textbf{57.2} & 26.3 & 59.4 & 62.4 & 69.6 & 47.6 & 81.2 & 77.9 & 63.5 & 68.4 & 53.6 & 49.6 & 0.3 & 78.6 & 71.0 & 43.0 & 70.1 & 26.5 & 32.4 & 61.2 \\
% Phang et. al & 68.6 & 53.2 & 57.8 & 60.8 & 61.0 & 69.3 & 54.2 & 83.8 & 80.8 & 69.4 & 70.6 & 58.9 & 53.7 & 2.2 & 75.2 & 77.2 & 57.7 & 75.6 & 46.1 & 30.4 & 64.7 \\
XLM-R & \textbf{71.6} & 56.2 & \textbf{60.0} & \textbf{67.8} & \textbf{68.1} & 57.1 & \textbf{54.3} & 84.0 & 81.9 & 69.1 & 70.5 & \textbf{59.5} & 55.8 & 1.3 & 73.2 & \textbf{76.1} & 56.4 & 79.4 & 33.6 & 33.1 & 65.4 \\
mT5-Small & 53.2 & 23.4 & 26.6 & 39.4 & 39.4 & 70.0 & 30.1 & 75.4 & 70.8 & 46.5 & 54.8 & 37.5 & 32.6 & 7.2 & 69.4 & 56.0 & 26.4 & 63.8 & 58.8 & 37.9 & 51.0 \\
mT5-Base & 50.1 & 23.4 & 33.9 & 48.2 & 43.8 & 72.6 & 37.0 & 80.1 & 76.0 & 55.4 & 62.4 & 41.2 & 42.7 & 9.5 & 74.6 & 58.4 & 38.4 & 73.0 & 59.3 & 41.5 & 56.6 \\
mT5-Large & 58.2 & 23.3 & 36.2 & 46.3 & 46.5 & 69.4 & 32.2 & 82.7 & 79.6 & 50.2 & 72.4 & 46.4 & 44.5 & \textbf{10.5} & 79.0 & 65.1 & 44.2 & 77.1 & 48.4 & 44.0 & 58.8 \\
mT5-XL & 66.0 & 31.6 & 38.1 & 54.1 & 57.6 & 74.8 & 42.6 & 85.7 & 85.2 & 66.9 & 72.8 & 49.0 & 54.7 & 9.6 & 84.1 & 67.7 & 64.7 & 79.6 & 59.9 & 54.4. & 65.7 \\
mT5-XXL & 66.0 & 38.7 & 43.5 & 54.5 & 63.1 & \textbf{77.6} & 44.7 & \textbf{87.7} & \textbf{86.9} & \textbf{72.0} & \textbf{72.9} & 56.5 & \textbf{59.5} & 10.4 & \textbf{85.2} & 71.4 & \textbf{80.7} & \textbf{84.6} & \textbf{70.0} & \textbf{56.8} & \textbf{69.2} \\
\bottomrule
\end{tabular}
\caption{WikiAnn NER F1 scores for each language.}
\end{table*}

==> results/pawsx.tex <==
\begin{table*}[h!]
\centering
\footnotesize
% Manually specify the width of the last column. Otherwise the last column is too wide.
\begin{tabular}{l|p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}p{3em}<{\centering}|p{3em}<{\centering\arraybackslash}}
\toprule
Model & en & de & es & fr & ja & ko & zh & avg \\
\midrule
\multicolumn{9}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 94.0& 85.7& 87.4& 87.0& 73.0& 69.6& 77.0 & 81.9 \\
XLM & 94.0& 85.9& 88.3& 87.4& 69.3& 64.8& 76.5 & 80.9 \\
%MMTE & 93.1& 85.1& 87.2& 86.9& 72.0& 69.2& 75.9 & 81.3 \\
XLM-R & 94.7& 89.7& 90.1& 90.4& 78.7& 79.0& 82.3 & 86.4 \\
%\textsc{Filter} & 96.5 & 92.5 & 93.0 & 93.8 & 86.7 & 87.1 & 88.3 & 91.2 \\
mT5-Small           & 92.2 & 86.2 & 86.1 & 86.6 & 74.7 & 73.5 & 77.9 & 82.4 \\
mT5-Base            & 95.4 & 89.4 & 89.6 & 91.2 & 79.8 & 78.5 & 81.1 & 86.4 \\
mT5-Large           & 96.1 & 91.3 & 92.0   & \textbf{92.7} & 82.5 & 82.7 & 84.7 & 88.9 \\
mT5-XL              & 96.0   & 92.8 & \textbf{92.7} & 92.4 & 83.6 & 83.1 & 86.5 & 89.6 \\
%mT5-XXL (75\%)      & 95.7 & 91.6 & 91.6 & 92.3 & 83.4 & 82.9 & \textbf{86.8} & 89.2 \\
mT5-XXL & \textbf{96.3} & \textbf{92.9} & 92.6 & \textbf{92.7} & \textbf{84.5} & \textbf{83.9} & \textbf{87.2} & \textbf{90.0} \\
\midrule
\multicolumn{9}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%\textsc{Filter} + Self-Teaching & 95.9 & 92.8 & 93.0 & 93.7 & \textbf{87.4} & 87.6 & 89.6 & 91.4 \\
mT5-Small & 87.9 & 81.4 & 83.1 & 84.1 & 74.2 & 71.7 & 76.7 & 79.9 \\
mT5-Base & 95.5 & 90.9 & 91.4 & 92.5 & 83.6 & 84.8 & 86.4 & 89.3 \\
mT5-Large & 96.4 & 92.7 & 93.3 & 93.6 & 86.5 & 87.4 & 88.4 & 91.2 \\
mT5-XL & 96.4 & 92.5 & 93.1 & 93.6 & 85.5 & 86.9 & \textbf{89.0} & 91.0 \\
mT5-XXL & \textbf{96.1} & \textbf{92.9} & \textbf{93.6} & \textbf{94.2} & \textbf{87.0} & \textbf{87.9} & \textbf{89.0} & \textbf{91.5} \\
\bottomrule
\end{tabular}
\caption{PAWS-X accuracy scores for each language.}
%\vspace{-3mm}
\end{table*}

==> results/tydiqa.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccc|c}
\toprule
Model &  en & ar & bn & fi & id & ko & ru & sw & te & avg \\

\midrule
\multicolumn{8}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule

mBERT & 75.3 / 63.6 &  62.2 / 42.8 &  49.3 / 32.7 &  59.7 / 45.3 &  64.8 / 45.8 &  58.8 / 50.0 &  60.0 / 38.8 &  57.5 / 37.9 &  49.6 / 38.4 &  59.7 / 43.9 \\
XLM & 66.9 / 53.9 &  59.4 / 41.2 &  27.2 / 15.0 &  58.2 / 41.4 &  62.5 / 45.8 &  14.2 / 5.1 &  49.2 / 30.7 &  39.4 / 21.6 &  15.5 / 6.9 &  43.6 / 29.1 \\
%MMTE & 62.9 / 49.8 &  63.1 / 39.2 &  55.8 / 41.9 &  53.9 / 42.1 &  60.9 / 47.6 &  49.9 / 42.6 &  58.9 / 37.9 &  63.1 / 47.2 &  54.2 / 45.8 &  58.1 / 43.8 \\
XLM-R & 71.5 / 56.8 &  67.6 / 40.4 &  64.0 / 47.8 &  70.5 / 53.2 &  77.4 / 61.9 &  31.9 / 10.9 &  67.0 / 42.1 &  66.1 / 48.1 &  70.1 / 43.6 &  65.1 / 45.0 \\
%\textsc{Filter} & 71.9 / 58.9 & 73.7 / 47.9 & 68.7 / 53.1 & 71.2 / 54.9 & 77.9 / 59.8 & 33.0 / 12.3 & 68.7 / 45.9 & 78.7 / 66.1 & 69.4 / 48.6 & 68.1 / 49.7 \\
mT5-Small & 53.9 / 43.6 & 41.1 / 26.0 & 18.9 / 13.3 & 39.2 / 22.6 & 44.4 / 31.7 & 24.9 / 16.3 & 40.5 / 24.3 & 34.8 / 21.2 & 16.9 / 11.5 & 34.9 / 23.4 \\
mT5-Base & 71.8 / 60.9 & 67.1 / 50.4 & 40.7 / 22.1 & 67.0 / 52.2 & 71.3 / 54.5 & 49.5 / 37.7 & 54.9 / 32.6 & 60.4 / 43.9 & 40.6 / 31.1 & 58.1 / 42.8 \\
mT5-Large & 71.6 / 58.9 & 60.5 / 40.4 & 42.0 / 23.9 & 64.6 / 48.8 & 67.0 / 49.2 & 47.6 / 37.3 & 58.9 / 36.8 & 65.7 / 45.3 & 41.9 / 29.7 & 57.8 / 41.2 \\
mT5-XL & 80.3 / 70.9 & 81.7 / 65.5 & 74.5 / 57.5 & 79.4 / 65.3 & 83.5 / 70.4 & 70.0 / 60.5 & 71.6 / 47.8 & 77.3 / 59.7 & 77.9 / 55.8 & 77.4 / 61.5 \\
%mT5-XXL (75\%) & \textbf{83.1} / \textbf{72.3}	& \textbf{83.3} / \textbf{67.2}	&	\textbf{80.9} / \textbf{68.1}	&	\textbf{82.9} / \textbf{70.2}	&	\textbf{86.3} / \textbf{75.6}	&	\textbf{73.7} / \textbf{63.0}	&	\textbf{75.2} / \textbf{53.8}	&	\textbf{82.4} / \textbf{66.5}	&	\textbf{79.2} / \textbf{59.6}	&	\textbf{80.8} / \textbf{66.3} \\
mT5-XXL & \textbf{83.7 / 72.5} & \textbf{82.8 / 66.0} & \textbf{80.2 / 63.7} & \textbf{83.3 / 70.2} & \textbf{85.3 / 73.3} & \textbf{76.2 / 64.1} & \textbf{76.6 / 55.8} & \textbf{81.9 / 66.1} & \textbf{79.2 / 58.7} & \textbf{81.0 / 65.6} \\

\midrule
\multicolumn{8}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule

%\textsc{Filter} + Self-Teaching & 72.4 / 59.1 & 72.8 / 50.8 & 70.5 / 56.6 & 73.3 / 57.2 & 76.8 / 59.8 & 33.1 / 12.3 & 68.9 / 46.6 & 77.4 / 65.7 & 69.9 / 50.4 & 68.3 / 50.9 \\
mT5-Small & 57.1 / 46.6 & 56.8 / 39.7 & 37.2 / 21.2 & 50.9 / 37.2 & 60.1 / 45.1 & 40.4 / 29.3 & 50.7 / 33.6 & 51.5 / 35.3 & 29.3 / 18.1 & 48.2 / 34.0 \\
mT5-Base & 71.1 / 58.9 & 68.0 / 50.2 & 57.4 / 35.4 & 68.8 / 55.2 & 73.5 / 57.2 & 56.5 / 43.8 & 64.0 / 45.8 & 65.8 / 48.3 & 51.2 / 34.1 & 64.0 / 47.7 \\
mT5-Large & 75.6 / 62.7 & 74.8 / 57.9 & 65.0 / 46.0 & 72.3 / 57.5 & 78.7 / 63.5 & 66.4 / 53.6 & 70.9 / 50.5 & 74.0 / 56.7 & 62.0 / 45.1 & 71.1 / 54.9 \\
mT5-XL & 82.0 / 65.7 &	79.3 / 65.5 &	80.4 / 68.9 &	79.1 / 64.7 &	84.7 / 71.0 &	70.5 / 56.2 &	78.3 / 61.1 &	83.9 / 70.9 &	80.9 / 64.0 &	79.9 / 65.3 \\
mT5-XXL & \textbf{83.3 / 71.6} & \textbf{83.0 / 66.3} & \textbf{82.3 / 70.8} & \textbf{82.9 / 67.8} & \textbf{86.6 / 72.0} & \textbf{75.0 / 62.3} & \textbf{80.7 / 63.1} & \textbf{86.9 / 75.8} & \textbf{84.6 / 69.2} & \textbf{82.8 / 68.8} \\

\midrule
\multicolumn{8}{l}{\emph{In-language multitask (models fine-tuned on gold data in all target languages)}} \\
\midrule

mT5-Small & 66.4 / 56.1	& 80.3 / 68.7 & 71.7 / 60.2 & 71.9 / 59.5 & 78.8 / 67.6 & 55.5 / 46.7 & 70.1 / 57.1 & 77.7 / 68.9 & 82.7 / 71.6 & 73.0 / 62.0 \\
mT5-Base & 76.6 / 65.2 & 84.2 / 71.8 & 80.0 / 69.0 & 80.1 / 69.3 & 85.5 / 75.0 & 70.3 / 61.6 & 77.5 / 64.4 & 83.6 / 74.9 & 88.2 / 78.0 & 80.8 / 70.0 \\
mT5-Large & 82.4 / 70.9 & 87.1 / 75.1 & 86.3 / 78.8 & 85.5 / 73.4 & 87.3 / 77.9 & 79.1 / 69.9 & 84.3 / 71.3 & 87.4 / 79.6 & 90.2 / 81.2 & 85.5 / 75.3 \\
mT5-XL & 84.1 / 74.3 & \textbf{88.5} / 76.0 & 87.7 / \textbf{80.5} & 87.4 / 76.1 & 89.9 / 81.2 & 82.8 / 75.4 & 84.9 / 73.2 & 90.1 / 82.8 & 92.0 / 83.7 & 87.5 / 78.1 \\
mT5-XXL & \textbf{85.7 / 75.5} & 88.4 / \textbf{76.9} & \textbf{88.7 / 80.5} & \textbf{87.5 / 76.3} & \textbf{90.3 / 81.8} & \textbf{83.7 / 75.7} & \textbf{87.9 / 76.8} & \textbf{91.9 / 84.4} & \textbf{92.6 / 83.9} & \textbf{88.5 / 79.1} \\

\bottomrule
\end{tabular}
\caption{TyDi QA GoldP results (F1/EM) for each language.}
%\vspace{-3mm}
\end{table*}





==> results/xnli.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccccccc|c}
\toprule
Model & en & ar & bg & de & el & es & fr & hi & ru & sw & th & tr & ur & vi & zh & avg \\
\midrule
\multicolumn{17}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule

mBERT &80.8& 64.3& 68.0& 70.0& 65.3& 73.5& 73.4& 58.9& 67.8& 49.7& 54.1& 60.9& 57.2& 69.3& 67.8& 65.4 \\
XLM &82.8& 66.0& 71.9& 72.7& 70.4& 75.5& 74.3& 62.5& 69.9& 58.1& 65.5& 66.4& 59.8& 70.7& 70.2& 69.1 \\
XLM-R &88.7& 77.2& 83.0& 82.5& 80.8& 83.7& 82.2& 75.6& 79.1& 71.2& 77.4& 78.0& 71.7& 79.3& 78.2& 79.2 \\
mT5-Small & 79.6 & 65.2 & 71.3 & 69.2 & 68.6  & 72.7 & 70.7 & 62.5 & 70.1 & 59.7 & 66.3 & 64.4 & 59.9 & 66.3 & 65.8 & 67.5 \\
mT5-Base & 84.7 & 73.3 & 78.6 & 77.4 & 77.1  & 80.3 & 79.1 & 70.8 & 77.1 & 69.4 & 73.2 & 72.8 & 68.3 & 74.2 & 74.1 & 75.4 \\
mT5-Large & 89.4 & 79.8 & 84.1 & 83.4 & 83.2  & 84.2 & 84.1 & 77.6 & 81.5 & 75.4 & 79.4 & 80.1 & 73.5 & 81.0 & 80.3 & 81.1 \\
mT5-XL & 90.6 & 82.2 & 85.4 & 85.8 & 85.4  & 81.3 & 85.3 & 80.4 & 83.7 & 78.6 & 80.9 & 82.0 & 77.0 & 81.8 & 82.7 & 82.9 \\
%mT5-XXL (75\%) & \textbf{92.3} & \textbf{84.4}& \textbf{87.5}& \textbf{87.3}& \textbf{87.0}&  \textbf{88.3}& \textbf{87.3}& \textbf{82.5}& \textbf{84.3}& \textbf{80.4}& \textbf{81.7}& \textbf{83.3}& \textbf{79.2}& \textbf{84.2}& \textbf{82.7}& \textbf{84.8}\\
mT5-XXL & \textbf{91.6} & \textbf{84.5} & \textbf{87.7} & \textbf{87.3} & \textbf{87.3} & \textbf{87.8} & \textbf{86.9} & \textbf{83.2} & \textbf{85.1} & \textbf{80.3} & \textbf{81.7} & \textbf{83.8} & \textbf{79.8} & \textbf{84.6} & \textbf{83.6} & \textbf{84.5} \\
\midrule
\multicolumn{17}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%Filter + Self-Teaching & 89.5 & 83.6 & 86.4 & 85.6 & 85.4 & 86.6 & 85.7 & 81.1 & 83.7 & 78.7 & 81.7 & 83.2 & 79.1 & 83.9 & 83.8 & 83.9 \\
mt5-Small & 69.5 & 63.7 & 67.5 & 65.7 & 66.4 & 67.5 & 67.3 & 61.9 & 66.4 & 59.6 & 63.9 & 63.5 & 60.4 & 63.3 & 64.5 & 64.7 \\
mt5-Base & 82.0 & 74.4 & 78.5 & 77.7 & 78.1 & 79.1 & 77.9 & 72.2 & 76.5 & 71.5 & 75.0 & 74.8 & 70.4 & 74.5 & 76.0 & 75.9 \\
mt5-Large & 88.3 & 80.3 & 84.1 & 84.0 & 83.7 & 84.9 & 83.8 & 79.8 & 82.0 & 76.4 & 79.9 & 81.0 & 75.9 & 81.3 & 81.7 & 81.8 \\
mt5-XL & 90.9 & 84.2 & 86.8 & 86.8 & 86.4 & 87.4 & 86.8 & 83.1 & 84.9 & 81.3 & 82.3 & 84.4 & 79.4 & 83.9 & 84.0 & 84.8 \\
mT5-XXL & \textbf{92.7} & \textbf{87.2} & \textbf{89.4} & \textbf{89.8} & \textbf{89.5} & \textbf{90.0} & \textbf{89.1} & \textbf{86.5} & \textbf{87.6} & \textbf{84.3} & \textbf{85.6} & \textbf{87.1} & \textbf{83.8} & \textbf{87.5} & \textbf{86.5} & \textbf{87.8} \\
\bottomrule
\end{tabular}
\caption{XNLI accuracy scores for each language.}
\end{table*}

==> results/xnli_ablation.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccccccc|c}
\toprule
Model & ar & bg & de & el & en & es & fr & hi & ru & sw & th & tr & ur & vi & zh & avg \\
\midrule
Baseline (mT5-large) & \textbf{79.8} & \textbf{84.1} & 83.4 & \textbf{83.2} & \textbf{89.4} & 84.2 & 84.1 & \textbf{77.6} & 81.5 & \textbf{75.4} & \textbf{79.4} & \textbf{80.1} & 73.5 & \textbf{81.0} & \textbf{80.3} & \textbf{81.1} \\
Dropout $0.1$ & 76.4 & 82.1 & 81.7 & 81.0 & 88.0 & 70.8 & 80.3 & 74.4 & 79.0 & 72.3 & 75.8 & 75.9 & 70.6 & 78.6 & 76.5 & 77.6 \\
Sequence length $512$ & 78.1 & 83.4 & 83.1 & 82.1 & 88.8 & 84.5 & 82.8 & 77.3 & 81.2 & \textbf{75.4} & 78.2 & 79.6 & 73.8 & 80.0 & 78.9 & 80.5 \\
Span length $10$ & 77.6 & 81.5 & 80.5 & 81.2 & 87.2 & 83.0 & 81.2 & 74.7 & 79.8 & 73.6 & 76.7 & 75.9 & 71.3 & 78.6 & 76.5 & 78.6 \\
$\alpha = 0.7$ & 79.3 & \textbf{84.1} & \textbf{84.5} & 83.1 & \textbf{89.4} & \textbf{85.3} & \textbf{84.4} & 76.4 & \textbf{82.8} & 70.6 & 78.7 & 79.8 & 71.7 & 80.3 & 79.9 & 80.7 \\
$\alpha = 0.2$ & 78.7 &83.8 &83.3 &82.5 &89.3 &83.4 &83.6 &77.3 &81.2 &\textbf{75.4} &78.6 &79.4 &\textbf{73.9} &79.9 &79.7 &80.7 \\
No line length filter & 78.4 & 83.3 & 81.5 & 81.4 & 88.9 & 83.8 & 82.5 & 74.4 & 80.5 & 69.4 & 77.6 & 76.9 & 71.3 & 78.8 & 78.3 & 79.1 \\
Add Wikipedia data & 79.3& 83.1& 83.1& 82.7& 88.6& 80.1& 83.2& 77.3& 81.4& 75.0& 78.9& 79.3& 73.5& 80.2& 79.2& 80.3\\
% Finetune 2M steps &79.7& 84.3& 83.7& 83.3& 89.3& 85.1& 84.1& 77.5& 81.9& 75.5& 79.1& 79.4& 74.3& 81.5& 79.6& 81.2 \\
% Train 2M dropout & 73.4& 79.0& 79.3& 77.7& 86.0& 62.5& 72.4& 71.6& 76.1& 69.1& 72.6& 68.9& 67.2& 75.1& 73.8& 73.7 \\
\bottomrule
\end{tabular}
\caption{XNLI zero-shot accuracy of various ablations on our mT5-Large model.}
\end{table*}

==> results/xquad.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccc|c}
\toprule
Model & en & ar & de & el & es & hi & ru & th & tr & vi & zh & avg \\
\midrule
\multicolumn{8}{l}{\emph{Cross-lingual zero-shot transfer (models fine-tune on English data only)}} \\
\midrule
mBERT & 83.5 / 72.2 &  61.5 / 45.1 &  70.6 / 54.0 &  62.6 / 44.9 &  75.5 / 56.9 &  59.2 / 46.0 &  71.3 / 53.3 &  42.7 / 33.5 &  55.4 / 40.1 &  69.5 / 49.6 &  58.0 / 48.3 &  64.5 / 49.4 \\
XLM & 74.2 / 62.1 &  61.4 / 44.7 &  66.0 / 49.7 &  57.5 / 39.1 &  68.2 / 49.8 &  56.6 / 40.3 &  65.3 / 48.2 &  35.4 / 24.5 &  57.9 / 41.2 &  65.8 / 47.6 &  49.7 / 39.7 &  59.8 / 44.3 \\
%MMTE & 80.1 / 68.1 &  63.2 / 46.2 &  68.8 / 50.3 &  61.3 / 35.9 &  72.4 / 52.5 &  61.3 / 47.2 &  68.4 / 45.2 &  48.4 / 35.9 &  58.1 / 40.9 &  70.9 / 50.1 &  55.8 / 36.4 &  64.4 / 46.2 \\
XLM-R & 86.5 / 75.7 &  68.6 / 49.0 &  80.4 / 63.4 &  79.8 / 61.7 &  82.0 / 63.9 &  76.7 / 59.7 &  \textbf{80.1 / 64.3} &  74.2 / 62.8
&  75.9 / 59.3 &  79.1 / 59.0 &  59.3 / 50.0 &  76.6 / 60.8 \\
%\textsc{Filter} & 85.6 / 73.0 & 79.8 / 61.3 & 82.5 / 66.2 & 82.6 / 64.6 & 84.8 / 67.4 & 83.1 / 66.5 & 82.5 / 66.8 & 80.7 / 73.9 & 81.2 / 65.7 & 83.3 / 64.1 & 78.9 / 75.7 & 82.3 / 67.8 \\
mT5-Small & 78.5 / 66.1 & 51.4 / 34.0 & 63.8 / 45.9 & 53.8 / 33.4 & 67.0 / 50.3 & 47.8 / 34.5 & 50.5 / 30.1 & 54.0 / 44.5 & 55.7 / 38.9 & 58.1 / 41.3 & 58.9 / 48.7 & 58.1 / 42.5 \\
mT5-Base & 84.6 / 71.7 & 63.8 / 44.3 & 73.8 / 54.5 & 59.6 / 35.6 & 74.8 / 56.1 & 60.3 / 43.4 & 57.8 / 34.7 & 57.6 / 45.7 & 67.9 / 48.2 & 70.7 / 50.3 & 66.1 / 54.1 & 67.0 / 49.0 \\
mT5-Large & 88.4 / 77.3 & 75.2 / 56.7 & 80.0 / 62.9 & 77.5 / 57.6 & 81.8 / 64.2 & 73.4 / 56.6 & 74.7 / 56.9 & 73.4 / 62.0 & 76.5 / 56.3 & 79.4 / 60.3 & 75.9 / 65.5 & 77.8 / 61.5 \\
mT5-XL & 88.8 / 78.1 & 77.4 / 60.8 & 80.4 / 63.5 & 80.4 / 61.2 & 82.7 / 64.5 & 76.1 / 60.3 & 76.2 / 58.8 & 74.2 / 62.5 & 77.7 / 58.4 & 80.5 / 60.8 & 80.5 / 71.0 & 79.5 / 63.6 \\
%mT5-XXL (75\%) & \textbf{90.8} / \textbf{79.7} & \textbf{79.7} / \textbf{62.7} & \textbf{83.6} / \textbf{66.8} & \textbf{82.0} / \textbf{64.0} & \textbf{84.7} / \textbf{67.9} & \textbf{81.0} / \textbf{64.8} & \textbf{80.2} / 64.0 & 72.9 / 58.1 & \textbf{80.0} / \textbf{59.9} & \textbf{83.0} / \textbf{62.9} & \textbf{82.5} / \textbf{71.6} & \textbf{81.9} / \textbf{65.7} \\
mT5-XXL & \textbf{90.9 / 80.1} & \textbf{80.3 / 62.6} & \textbf{83.1 / 65.5} & \textbf{83.3 / 65.5} & \textbf{85.1 / 68.1} & \textbf{81.7 / 65.9} & 79.3 / 63.6 & \textbf{77.8 / 66.1} & \textbf{80.2 / 60.9} & \textbf{83.1 / 63.6} & \textbf{83.1 / 73.4} & \textbf{82.5 / 66.8}
 \\
\midrule
\multicolumn{8}{l}{\emph{Translate-train (models fine-tune on English training data plus translations in all target languages)}} \\
\midrule
%\textsc{Filter} + Self-Teaching & 86.4 / 74.6 & 79.5 / 60.7 & 83.2 / 67.0 & 83.0 / 64.6 & 85.0 / 67.9 & 83.1 / 66.6 & 82.8 / 67.4 & \textbf{79.6} / \textbf{73.2} & 80.4 / 64.4 & 83.8 / 64.7 & 79.9 / 77.0 & 82.4 / 68.0 \\
mT5-Small & 74.0 / 61.2 & 61.0 / 45.0 & 66.0 / 50.2 & 64.1 / 47.2 & 67.5 / 50.8 & 60.2 / 43.7 & 64.4 / 46.7 & 58.9 / 52.9 & 59.0 / 39.4 & 63.5 / 46.0 & 68.2 / 61.2 & 64.3 / 49.5 \\
mT5-Base & 83.1 / 70.3 & 72.4 / 55.2 & 76.9 / 59.7 & 76.8 / 58.8 & 79.0 / 61.2 & 71.4 / 53.4 & 76.1 / 58.5 & 67.9 / 62.0 & 72.5 / 51.4 & 75.9 / 56.3 & 76.9 / 69.7 & 75.3 / 59.7 \\
mT5-Large & 87.3 / 75.5 & 79.4 / 62.7 & 82.7 / 66.0 & 81.8 / 63.5 & 83.8 / 66.1 & 78.0 / 59.8 & 81.9 / 66.3 & 74.7 / 68.2 & 80.2 / 59.2 & 80.4 / 60.8 & 83.2 / 76.9 & 81.2 / 65.9 \\
mT5-XL & 88.5 / 77.1 & 80.9 / 65.4 & 83.4 / 66.7 & 83.6 / 64.9 & 84.9 / 68.2 & 79.6 / 63.1 & 82.7 / 67.1 & 78.5 / 72.9 & 82.4 / 63.8 & 82.4 / 64.1 & 83.2 / 75.9 & 82.7 / 68.1 \\
mT5-XXL & \textbf{91.3 / 80.3} &	\textbf{83.4 / 68.2} &	\textbf{85.0 / 68.2} &	\textbf{85.9 / 68.9} &	\textbf{87.4 / 70.8} &	\textbf{83.7 / 68.2} &	\textbf{85.2 / 70.4} &	\textbf{80.2 / 74.5} &	\textbf{84.4 / 67.7} &	\textbf{85.3 / 67.1} &	\textbf{85.7 / 80.0} &	\textbf{85.2 / 71.3} \\
\bottomrule
\end{tabular}
\caption{XQuAD results (F1/EM) for each language.}
%\vspace{-3mm}
\end{table*}

==> results/xquad_ablation.tex <==
\begin{table*}[h!]
\centering
\footnotesize
\begin{tabular}{l|ccccccccccc|c}
\toprule   
Model & en & ar & de & el & es & hi & ru & th & tr & vi & zh & avg \\
\midrule
Baseline(mT5-large) & 88.4 / 77.3    & 75.2 / 56.7    & 80.0 / \textbf{62.9}    & 77.5 / 57.6    & \textbf{81.8} / 64.2    & 73.4 / 56.6    & 74.7 / 56.9    & 73.4 / \textbf{62.0}    & 76.5 / 56.3    & 79.4 / \textbf{60.3}    & 75.9 / 65.5 & 77.8 / 61.5 \\
Span length $10$   & 88.1 / 76.3   & 70.0 / 50.6   & 78.1 / 60.2   & 68.8 / 44.0   & 79.0 / 60.8   & 67.3 / 48.4   & 65.4 / 43.3   & 68.1 / 57.2   & 74.4 / 53.6   & 77.9 / 57.7   & 76.6 / 66.4   & 74.0 / 56.2   \\
Dropout $0.1$   & 87.3 / 76.0   & 54.9 / 33.9   & 77.6 / 60.2   & 64.4 / 40.1   & 79.2 / 60.6   & 59.1 / 40.4   & 59.5 / 38.4   & 65.7 / 51.0   & 73.6 / 52.8   & 75.8 / 55.8   & 77.0 / 64.5   & 70.4 / 52.1   \\
Sequence length $512$  & 88.0 / 76.9   & \textbf{77.0} / 59.6   & 80.2 / 62.4   & \textbf{79.8} / \textbf{60.0}   & 81.7 / \textbf{64.4}   & \textbf{75.1} / \textbf{57.5}   & \textbf{77.4} / \textbf{58.5}   & 72.7 / 59.8   & 75.3 / 53.9   & 79.4 / 58.9   & 78.5 / 67.2   & \textbf{78.6} / \textbf{61.7}   \\
$\alpha = 0.7$  & 88.4 / 77.1   & 76.5 / 58.8   & 78.5 / 59.8   & 77.2 / 55.5   & 78.7 / 59.5   & 74.6 / 56.8   & 73.1 / 54.5   & 72.5 / 60.2   & 75.7 / 55.0   & 79.2 / 58.3   & \textbf{78.6} / 66.2   & 77.5 / 60.2   \\
 $\alpha = 0.2$  & 87.9 / 76.8   & 75.5 / 57.3   & 80.2 / 62.4   & 76.2 / 54.0   & 81.6 / 63.7   & 73.7 / 57.0   & 70.7 / 50.8   & 72.2 / 60.4   & 75.5 / 55.7   & \textbf{79.7} / 59.7   & 78.3 / \textbf{67.5}   & 77.4 / 60.5   \\
No line length filter & 88.9 / 77.4   & 73.8 / 54.0   & \textbf{80.8} / 62.7   & 74.2 / 51.8   & 80.9 / 62.8   & 74.1 / 56.6   & 75.0 / 56.4   & 71.7 / 60.3   & \textbf{76.7} / 56.0   & 78.8 / 58.6   & 78.5 / 67.1   & 77.6 / 60.3   \\
 Add Wikipedia data    & \textbf{89.3} / \textbf{78.4}   & 69.6 / 48.9   & 79.6 / 61.1   & 59.5 / 36.0   & 80.6 / 61.0   & 73.6 / 55.0   & 68.7 / 47.0   & 70.5 / 58.1   & \textbf{76.7} / \textbf{56.9}   & 78.6 / 56.4   & 77.5 / 66.3   & 74.9 / 56.8   \\
% Finetune 2M steps       & 37.5 / 22.7   & 75.7 / \textbf{63.9}   & 58.0 / 38.8   & 58.9 / 42.2   & 62.6 / 45.9   & 32.3 / 21.3   & 31.2 / 17.4   & 60.2 / 50.5   & 50.2 / 33.1   & 58.1 / 39.7   & 39.5 / 31.6   & 51.3 / 37.0  \\

\bottomrule
\end{tabular}
\caption{XQuAD zero-shot F1/EM of various ablations on our mT5-Large model.}
\end{table*}
